Private Speech Classification with Secure Multiparty Computation

Deep learning in audio signal processing, such as human voice audio signal classification, is a rich application area of machine learning. Legitimate use cases include voice authentication, gunfire detection, and emotion recognition. While there are clear advantages to automated human speech classification, application developers can gain knowledge beyond the professed scope from unprotected audio signal processing. In this paper we propose the first privacy-preserving solution for deep learning-based audio classification that is provably secure. Our approach, which is based on Secure Multiparty Computation, allows to classify a speech signal of one party (Alice) with a deep neural network of another party (Bob) without Bob ever seeing Alice's speech signal in an unencrypted manner. As threat models, we consider both passive security, i.e. with semi-honest parties who follow the instructions of the cryptographic protocols, as well as active security, i.e. with malicious parties who deviate from the protocols. We evaluate the efficiency-security-accuracy trade-off of the proposed solution in a use case for privacy-preserving emotion detection from speech with a convolutional neural network. In the semi-honest case we can classify a speech signal in under 0.3 sec; in the malicious case it takes $\sim$1.6 sec. In both cases there is no leakage of information, and we achieve classification accuracies that are the same as when computations are done on unencrypted data.

==> Private Speech Classification with Secure Multiparty Computation/header.tex <==
% --- -----------------------------------------------------------------
% --- Packages
% --- -----------------------------------------------------------------

\usepackage{longtable}
\usepackage{latexsym}
\usepackage{amscd}
\usepackage{amsfonts}
\usepackage{float}
\usepackage{longtable}
\usepackage{xspace}
\usepackage{stmaryrd}
\usepackage[utf8]{inputenc}



% --- -----------------------------------------------------------------
% --- Other Formatting Definitions
% --- -----------------------------------------------------------------



\DeclareMathAlphabet{\mathsl}{OT1}{cmr}{m}{sl}
\DeclareMathAlphabet{\mathsc}{OT1}{cmr}{m}{sc}
\DeclareMathAlphabet{\mathslbf}{OT1}{cmr}{bx}{sl}
% math script font; extra commands to make slightly larger
\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}%
             {<-> s * [1.150] pzcmi7t}{}
\DeclareMathAlphabet{\mathscript}{OT1}{pzc}{m}{it}


% --- -----------------------------------------------------------------
% --- Theorems Environments
% --- -----------------------------------------------------------------

\newenvironment{definition}{\begin{defn}}{\end{defn}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{propo}[thm]{Proposition}
\newtheorem{clm}[thm]{Claim}
\newtheorem{defn}[thm]{Definition}
\newtheorem{assm}[thm]{Assumption}
\newtheorem{rem}[thm]{Remark}
\newtheorem{obs}[thm]{Observation}
\newtheorem{egs}[thm]{Example}
\newtheorem{expr}{Experiment}
\newtheorem{fct}[thm]{Fact}
\newtheorem{cons}[thm]{Construction}
\newtheorem{nte}[thm]{Note}
\newtheorem{protocol}[thm]{Protocol}
\newtheorem{prop}[thm]{Properties}





\newcommand{\charef}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\apref}[1]{Appendix~\ref{#1}}
\newcommand{\thref}[1]{Theorem~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\clref}[1]{Claim~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\factref}[1]{Fact~\ref{#1}}
\newcommand{\remref}[1]{Remark~\ref{#1}}
\newcommand{\obsref}[1]{Observation~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{Construction~\ref{#1}}

\newenvironment{sfigure}{\begin{figure}[t]\begin{small}}{\end{small}\end{figure}}
\def\figurewidth{0.97\columnwidth}

%\newcommand{\widthfigure}[3]{\begin{figure}\begin{tabular}{p{\figurewidth}}#1\end{tabular}\vspace{-0.1in}\caption{#2.}\label{#3}\end{figure}}

\newcommand{\widthfigure}[3]{\begin{figure}\begin{center}\begin{tabular}{|p{\figurewidth}|}\hline#1\hline\end{tabular}\end{center}\smallskip\caption{#2.}\label{#3}\end{figure}}


\newcommand{\widthtable}[4]{\begin{table*}[!ht]\centering
\begin{tabular}{#1}#2\end{tabular}\smallskip\caption{#3.}\label{#4}\end{table*}}

%\newcommand{\widthtable}[4]{\begin{table*}\centering\resizebox{\textwidth}{!}{\begin{tabular}{#1}#2\end{tabular}}\smallskip\caption{#3.}\label{#4}\end{table*}}







% --- -----------------------------------------------------------------
% --- Proof Environment
% --- -----------------------------------------------------------------




% --- -----------------------------------------------------------------
% --- General Macros (not specific to this paper)
% --- -----------------------------------------------------------------

% authors notes
\newcommand{\authnote}[2]{
\ifnum\authnotes=1 
  \begin{center}
    \fbox{\begin{minipage}{5.7in}
      \textbf{#1 says:} #2
    \end{minipage}}
  \end{center} 
\fi
}



% assumptions
\def\CDH{\textrm{CDH}\xspace}
\def\coCDH{\textrm{co-CDH}\xspace}
\def\XCDHI{\textrm{XDHI}\xspace}
\def\DLIN{\textrm{DLIN}\xspace}
\def\SDP{\textrm{SDP}\xspace}
\def\SFP{\textrm{SFP}\xspace}
\def\kSFP{$\k$-\textrm{SFP}\xspace}
\def\STP{\textrm{STP}\xspace}
\def\DPA{\textrm{DBP}\xspace}
\def\DDH{\textrm{DDH}\xspace}
\def\DDHl{\text{$\textrm{DDH}_{1}$}\xspace}
\def\DDHr{\text{$\textrm{DDH}_{2}$}\xspace}
\def\DPAl{\text{$\DPA_1$}\xspace}
\def\DPAr{\text{$\DPA_2$}\xspace}
\def\XDDH{\textrm{XDDH}\xspace}
\def\SXDH{\textrm{SXDH}\xspace}
\def\SDL{\textrm{XDLIN}\xspace}
\def\XDLIN{\textrm{XDLIN}\xspace}
\def\XDLINl{\text{$\textrm{XDLIN}_{1}$}\xspace}
\def\XDLINr{\text{$\textrm{XDLIN}_{2}$}\xspace}
\def\SXDLIN{\textrm{SXDLIN}\xspace}
\def\DLINl{\text{$\textrm{DLIN}_{1}$}\xspace}
\def\DLINr{\text{$\textrm{DLIN}_{2}$}\xspace}

\def\cdh{\textsf{cdh}\xspace}
\def\cocdh{\textsf{co-cdh}\xspace}
\def\xcdi{\textsf{xdhi}\xspace}
\def\dlin{\textsf{dlin}\xspace}
\def\sdp{\textsf{sdp}\xspace}
\def\sfp{\textsf{sfp}\xspace}
\def\ksfp{$\k$-\textsf{sfp}\xspace}
\def\stpa{\textsf{stp}\xspace}
\def\dpa{\textsf{dbp}\xspace}
\def\ddh{\textsf{ddh}\xspace}
\def\ddhl{\textsf{{\ddh}1}\xspace}
\def\ddhr{\textsf{{\ddh}2}\xspace}
\def\dpal{\textsf{{\dpa}1}\xspace}
\def\dpar{\textsf{{\dpa}2}\xspace}
\def\xddh{\textsf{xddh}\xspace}
\def\sxdh{\textsf{sxdh}\xspace}
\def\sdl{\textsf{xdlin}\xspace}
\def\xdlin{\textsf{xdlin}\xspace}
\def\xdlinl{\textsf{{\xdlin}1}\xspace}
\def\xdlinr{\textsf{{\xdlin}2}\xspace}
\def\sxdlin{\textsf{sxdlin}\xspace}
\def\dlinl{\textsf{{\dlin}1}\xspace}
\def\dlinr{\textsf{{\dlin}2}\xspace}


% calligraphic letters
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}


% vectors
\newcommand{\veca}{\mathbf{a}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecc}{\mathbf{c}}
\newcommand{\vecd}{\mathbf{d}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecf}{\mathbf{f}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vech}{\mathbf{h}}
\newcommand{\veci}{\mathbf{i}}
\newcommand{\vecj}{\mathbf{j}}
\newcommand{\veck}{\mathbf{k}}
\newcommand{\vecl}{\mathbf{l}}
\newcommand{\vecm}{\mathbf{m}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\veco}{\mathbf{o}}
\newcommand{\vecp}{\mathbf{p}}
\newcommand{\vecq}{\mathbf{q}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\vecs}{\mathbf{s}}
\newcommand{\vect}{\mathbf{t}}
\newcommand{\vecu}{\mathbf{u}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecz}{\mathbf{z}}
\newcommand{\vecbot}{\mathbf{\bot}}


% matrices
\newcommand{\mata}{\mathbf{A}}
\newcommand{\matb}{\mathbf{B}}
\newcommand{\matc}{\mathbf{C}}
\newcommand{\matd}{\mathbf{D}}
\newcommand{\mate}{\mathbf{E}}
\newcommand{\matf}{\mathbf{F}}
\newcommand{\matg}{\mathbf{G}}
\newcommand{\mati}{\mathbf{I}}
\newcommand{\matj}{\mathbf{J}}
\newcommand{\matk}{\mathbf{K}}
\newcommand{\matl}{\mathbf{L}}
\newcommand{\matm}{\mathbf{M}}
\newcommand{\matn}{\mathbf{N}}
\newcommand{\mato}{\mathbf{O}}
\newcommand{\matp}{\mathbf{P}}
\newcommand{\matq}{\mathbf{Q}}
\newcommand{\matr}{\mathbf{R}}
\newcommand{\mats}{\mathbf{S}}
\newcommand{\matt}{\mathbf{T}}
\newcommand{\matu}{\mathbf{U}}
\newcommand{\matv}{\mathbf{V}}
\newcommand{\matw}{\mathbf{W}}
\newcommand{\matx}{\mathbf{X}}
\newcommand{\maty}{\mathbf{Y}}
\newcommand{\matz}{\mathbf{Z}}


% sets
%\newcommand{\G}{{{\mathbb G}}}
\newcommand{\N}{{{\mathbb N}}}
\newcommand{\Z}{{{\mathbb Z}}}
\newcommand{\R}{{{\mathbb R}}}
\def\Zp{\mathbb{Z}_\p}
\def\Zps{\mathbb{Z}_\p^*}
\newcommand{\Fq}{\mathbb{F}_q} 
\def\bits{\{0,1\}}


% pairings
\def\pair{e}
\def\desc{\Lambda}
\def\descsym{\desc_{\textsf{sym}}}
\def\gorder{\p}
\def\Gl{\G_1} %base group in the left 
\def\Gr{\G_2} %base group in the right
\def\Gt{\G_T} %target group
\def\GlGen{G} %default generator in \Gl
\def\GrGen{\hat{G}} %default generator in \Gr
\def\GtGen{G_T} %default generator in \Gr
\def\Gls{\Gl^*}
\def\Grs{\Gr^*}
\def\Gs{\G^*}


% operations
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\condProb}[2]{{\Pr}\left[\,#1\,|\,#2\,\right]}
\newcommand{\expect}[1]{{{\mathbf{E}}[{#1}]}}
\newcommand{\infi}[2]{\inf_{#1}\left\{#2\right\}}
\newcommand{\supr}[2]{\sup_{#1}\left\{#2\right\}}
\newcommand{\ceiling}[1]{\lceil #1\rceil}
\newcommand{\inner}[2]{\langle{#1,#2}\rangle}
\def\pprod{{\textstyle\prod}}
\def\ssum{{\textstyle\sum}}
\newcommand{\sfrac}[2]{{\textstyle\frac{#1}{#2}}}
\def\cross{\times}
\def\union{\cup}
\def\bigunion{\bigcup}
\def\intersection{\cap}
\def\bigintersection{\bigcap}
\newcommand{\concat}{{\,\|\,}}
\newcommand{\xor}{{\;\oplus\;}}
\newcommand{\OR}{{\textstyle\bigvee}}
\newcommand{\AND}{\;\wedge\;}
\newcommand{\eqdef}{\;\stackrel{\rm def}{=}\;}
\def\getsr{\stackrel{{\scriptscriptstyle\$}}{\leftarrow}}
\newcommand{\goesto}{{\rightarrow}}
\newcommand{\then}{{\;;\;\;}}  
\newcommand{\andthen}{{\;:\;\;}}
\def\suchthatt{\: :\:}
\newcommand{\suchthat}{{\mbox{s.t.\ }}}
\def\next{\,;\,}
\newcommand{\Colon}{{:\;\;}}


% games
\newcommand{\procfont}[1]{\mathsc{#1}}
\newcommand{\Initialize}{\procfont{Initialize}}
\newcommand{\Finalize}{\procfont{Finalize}}
\newcommand{\Onquery}[2]{\underline{\procfont{#1}(#2)}}
\newcommand{\InitializeCode}[1]{\Onquery{Initialize}{#1}}
\newcommand{\FinalizeCode}[1]{\Onquery{Finalize}{#1}}
\newcommand{\EncO}{\procfont{Enc}}
\newcommand{\DecO}{\procfont{Dec}}
\newcommand{\procLR}{\procfont{LR}}
\newcommand{\outputs}{\textrm{ outputs }}
\newcommand{\wins}{\textrm{ wins}}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\bad}{\mathsf{bad}}


% cryptosystems
\newcommand{\secpar}{\lambda}
\newcommand{\pk}{\mathsl{pk}}
\newcommand{\sk}{\mathsl{sk}}
\newcommand{\enc}{\mathcal{E}}
\newcommand{\keys}{\mathcal{K}}
\newcommand{\decc}{\mathcal{D}}
\newcommand{\advA}{A}
%\newcommand{\msg}{\mathsl{m}}
\newcommand{\ciph}{\mathsl{c}}
\newcommand{\coins}[1]{\mathsf{coins(#1)}}
\newcommand{\reject}{\bot}


% --- -----------------------------------------------------------------
% --- Specific Macros
% --- -----------------------------------------------------------------
\newcommand{\peq}{\ensuremath{\pi_{\mathsf{EQ}}}\xspace}
\newcommand{\pfe}{\ensuremath{\pi_{\mathsf{FE}}}\xspace}
\newcommand{\pab}{\ensuremath{\pi_{\mathsf{AB}}}\xspace}
\newcommand{\plr}{\ensuremath{\pi_{\mathsf{LR}}}\xspace}
\newcommand{\pconv}{\ensuremath{\pi_{\mathsf{2toQ}}}\xspace}
\newcommand{\pmul}{\ensuremath{\pi_{\mathsf{DM}}}\xspace}
\newcommand{\pmmul}{\ensuremath{\pi_{\mathsf{DMM}}}\xspace}
\newcommand{\pip}{\ensuremath{\pi_{\mathsf{IP}}}\xspace}
\newcommand{\pcomp}{\ensuremath{\pi_{\mathsf{DC}}}\xspace}
\newcommand{\pdecomp}{\ensuremath{\pi_{\mathsf{decomp}}}\xspace}
\newcommand{\ptclr}{\ensuremath{\pi_{\mathsf{TC-LR}}}\xspace}
\newcommand{\ptcab}{\ensuremath{\pi_{\mathsf{TC-AB}}}\xspace}

\newcommand{\feq}{\ensuremath{\mathcal{F}_{\mathsf{EQ}}}\xspace}
\newcommand{\ffe}{\ensuremath{\mathcal{F}_{\mathsf{FE}}}\xspace}
\newcommand{\fab}{\ensuremath{\mathcal{F}_{\mathsf{AB}}}\xspace}
\newcommand{\flr}{\ensuremath{\mathcal{F}_{\mathsf{LR}}}\xspace}
\newcommand{\fconv}{\ensuremath{\mathcal{F}_{\mathsf{2toQ}}}\xspace}
\newcommand{\fmul}{\ensuremath{\mathcal{F}_{\mathsf{DM}}}\xspace}
\newcommand{\fmmul}{\ensuremath{\mathcal{F}_{\mathsf{DMM}}}\xspace}
\newcommand{\fcomp}{\ensuremath{\mathcal{F}_{\mathsf{DC}}}\xspace}
\newcommand{\fdecomp}{\ensuremath{\mathcal{F}_{\mathsf{decomp}}}\xspace}
\newcommand{\fti}[1]{\ensuremath{\mathcal{F}^{\mathcal{D}_{#1}}_{\mathsf{TI}}}\xspace}
\newcommand{\ftclr}{\ensuremath{\mathcal{F}_{\mathsf{TC-LR}}}\xspace}
\newcommand{\ftcab}{\ensuremath{\mathcal{F}_{\mathsf{TC-AB}}}\xspace}



\newcommand{\s}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\env}{\ensuremath{\mathcal{Z}}\xspace}
\newcommand{\adv}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\F}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\alice}{\ensuremath{\mathsf{A}}\xspace}
\newcommand{\bob}{\ensuremath{\mathsf{B}}\xspace}
\newcommand{\shareq}[1]{\ensuremath{\llbracket{#1}\rrbracket_{_q}}\xspace}
\newcommand{\sharetwo}[1]{\ensuremath{\llbracket{#1}\rrbracket_{_2}}\xspace}


==> header.tex <==
% --- -----------------------------------------------------------------
% --- Packages
% --- -----------------------------------------------------------------

\usepackage{longtable}
\usepackage{latexsym}
\usepackage{amscd}
\usepackage{amsfonts}
\usepackage{float}
\usepackage{longtable}
\usepackage{xspace}
\usepackage{stmaryrd}
\usepackage[utf8]{inputenc}



% --- -----------------------------------------------------------------
% --- Other Formatting Definitions
% --- -----------------------------------------------------------------



\DeclareMathAlphabet{\mathsl}{OT1}{cmr}{m}{sl}
\DeclareMathAlphabet{\mathsc}{OT1}{cmr}{m}{sc}
\DeclareMathAlphabet{\mathslbf}{OT1}{cmr}{bx}{sl}
% math script font; extra commands to make slightly larger
\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}%
             {<-> s * [1.150] pzcmi7t}{}
\DeclareMathAlphabet{\mathscript}{OT1}{pzc}{m}{it}


% --- -----------------------------------------------------------------
% --- Theorems Environments
% --- -----------------------------------------------------------------

\newenvironment{definition}{\begin{defn}}{\end{defn}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{propo}[thm]{Proposition}
\newtheorem{clm}[thm]{Claim}
\newtheorem{defn}[thm]{Definition}
\newtheorem{assm}[thm]{Assumption}
\newtheorem{rem}[thm]{Remark}
\newtheorem{obs}[thm]{Observation}
\newtheorem{egs}[thm]{Example}
\newtheorem{expr}{Experiment}
\newtheorem{fct}[thm]{Fact}
\newtheorem{cons}[thm]{Construction}
\newtheorem{nte}[thm]{Note}
\newtheorem{protocol}[thm]{Protocol}
\newtheorem{prop}[thm]{Properties}





\newcommand{\charef}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\apref}[1]{Appendix~\ref{#1}}
\newcommand{\thref}[1]{Theorem~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\clref}[1]{Claim~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\factref}[1]{Fact~\ref{#1}}
\newcommand{\remref}[1]{Remark~\ref{#1}}
\newcommand{\obsref}[1]{Observation~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{Construction~\ref{#1}}

\newenvironment{sfigure}{\begin{figure}[t]\begin{small}}{\end{small}\end{figure}}
\def\figurewidth{0.97\columnwidth}

%\newcommand{\widthfigure}[3]{\begin{figure}\begin{tabular}{p{\figurewidth}}#1\end{tabular}\vspace{-0.1in}\caption{#2.}\label{#3}\end{figure}}

\newcommand{\widthfigure}[3]{\begin{figure}\begin{center}\begin{tabular}{|p{\figurewidth}|}\hline#1\hline\end{tabular}\end{center}\smallskip\caption{#2.}\label{#3}\end{figure}}


\newcommand{\widthtable}[4]{\begin{table*}[!ht]\centering
\begin{tabular}{#1}#2\end{tabular}\smallskip\caption{#3.}\label{#4}\end{table*}}

%\newcommand{\widthtable}[4]{\begin{table*}\centering\resizebox{\textwidth}{!}{\begin{tabular}{#1}#2\end{tabular}}\smallskip\caption{#3.}\label{#4}\end{table*}}







% --- -----------------------------------------------------------------
% --- Proof Environment
% --- -----------------------------------------------------------------




% --- -----------------------------------------------------------------
% --- General Macros (not specific to this paper)
% --- -----------------------------------------------------------------

% authors notes
\newcommand{\authnote}[2]{
\ifnum\authnotes=1 
  \begin{center}
    \fbox{\begin{minipage}{5.7in}
      \textbf{#1 says:} #2
    \end{minipage}}
  \end{center} 
\fi
}



% assumptions
\def\CDH{\textrm{CDH}\xspace}
\def\coCDH{\textrm{co-CDH}\xspace}
\def\XCDHI{\textrm{XDHI}\xspace}
\def\DLIN{\textrm{DLIN}\xspace}
\def\SDP{\textrm{SDP}\xspace}
\def\SFP{\textrm{SFP}\xspace}
\def\kSFP{$\k$-\textrm{SFP}\xspace}
\def\STP{\textrm{STP}\xspace}
\def\DPA{\textrm{DBP}\xspace}
\def\DDH{\textrm{DDH}\xspace}
\def\DDHl{\text{$\textrm{DDH}_{1}$}\xspace}
\def\DDHr{\text{$\textrm{DDH}_{2}$}\xspace}
\def\DPAl{\text{$\DPA_1$}\xspace}
\def\DPAr{\text{$\DPA_2$}\xspace}
\def\XDDH{\textrm{XDDH}\xspace}
\def\SXDH{\textrm{SXDH}\xspace}
\def\SDL{\textrm{XDLIN}\xspace}
\def\XDLIN{\textrm{XDLIN}\xspace}
\def\XDLINl{\text{$\textrm{XDLIN}_{1}$}\xspace}
\def\XDLINr{\text{$\textrm{XDLIN}_{2}$}\xspace}
\def\SXDLIN{\textrm{SXDLIN}\xspace}
\def\DLINl{\text{$\textrm{DLIN}_{1}$}\xspace}
\def\DLINr{\text{$\textrm{DLIN}_{2}$}\xspace}

\def\cdh{\textsf{cdh}\xspace}
\def\cocdh{\textsf{co-cdh}\xspace}
\def\xcdi{\textsf{xdhi}\xspace}
\def\dlin{\textsf{dlin}\xspace}
\def\sdp{\textsf{sdp}\xspace}
\def\sfp{\textsf{sfp}\xspace}
\def\ksfp{$\k$-\textsf{sfp}\xspace}
\def\stpa{\textsf{stp}\xspace}
\def\dpa{\textsf{dbp}\xspace}
\def\ddh{\textsf{ddh}\xspace}
\def\ddhl{\textsf{{\ddh}1}\xspace}
\def\ddhr{\textsf{{\ddh}2}\xspace}
\def\dpal{\textsf{{\dpa}1}\xspace}
\def\dpar{\textsf{{\dpa}2}\xspace}
\def\xddh{\textsf{xddh}\xspace}
\def\sxdh{\textsf{sxdh}\xspace}
\def\sdl{\textsf{xdlin}\xspace}
\def\xdlin{\textsf{xdlin}\xspace}
\def\xdlinl{\textsf{{\xdlin}1}\xspace}
\def\xdlinr{\textsf{{\xdlin}2}\xspace}
\def\sxdlin{\textsf{sxdlin}\xspace}
\def\dlinl{\textsf{{\dlin}1}\xspace}
\def\dlinr{\textsf{{\dlin}2}\xspace}


% calligraphic letters
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}


% vectors
\newcommand{\veca}{\mathbf{a}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecc}{\mathbf{c}}
\newcommand{\vecd}{\mathbf{d}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecf}{\mathbf{f}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vech}{\mathbf{h}}
\newcommand{\veci}{\mathbf{i}}
\newcommand{\vecj}{\mathbf{j}}
\newcommand{\veck}{\mathbf{k}}
\newcommand{\vecl}{\mathbf{l}}
\newcommand{\vecm}{\mathbf{m}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\veco}{\mathbf{o}}
\newcommand{\vecp}{\mathbf{p}}
\newcommand{\vecq}{\mathbf{q}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\vecs}{\mathbf{s}}
\newcommand{\vect}{\mathbf{t}}
\newcommand{\vecu}{\mathbf{u}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecz}{\mathbf{z}}
\newcommand{\vecbot}{\mathbf{\bot}}


% matrices
\newcommand{\mata}{\mathbf{A}}
\newcommand{\matb}{\mathbf{B}}
\newcommand{\matc}{\mathbf{C}}
\newcommand{\matd}{\mathbf{D}}
\newcommand{\mate}{\mathbf{E}}
\newcommand{\matf}{\mathbf{F}}
\newcommand{\matg}{\mathbf{G}}
\newcommand{\mati}{\mathbf{I}}
\newcommand{\matj}{\mathbf{J}}
\newcommand{\matk}{\mathbf{K}}
\newcommand{\matl}{\mathbf{L}}
\newcommand{\matm}{\mathbf{M}}
\newcommand{\matn}{\mathbf{N}}
\newcommand{\mato}{\mathbf{O}}
\newcommand{\matp}{\mathbf{P}}
\newcommand{\matq}{\mathbf{Q}}
\newcommand{\matr}{\mathbf{R}}
\newcommand{\mats}{\mathbf{S}}
\newcommand{\matt}{\mathbf{T}}
\newcommand{\matu}{\mathbf{U}}
\newcommand{\matv}{\mathbf{V}}
\newcommand{\matw}{\mathbf{W}}
\newcommand{\matx}{\mathbf{X}}
\newcommand{\maty}{\mathbf{Y}}
\newcommand{\matz}{\mathbf{Z}}


% sets
%\newcommand{\G}{{{\mathbb G}}}
\newcommand{\N}{{{\mathbb N}}}
\newcommand{\Z}{{{\mathbb Z}}}
\newcommand{\R}{{{\mathbb R}}}
\def\Zp{\mathbb{Z}_\p}
\def\Zps{\mathbb{Z}_\p^*}
\newcommand{\Fq}{\mathbb{F}_q} 
\def\bits{\{0,1\}}


% pairings
\def\pair{e}
\def\desc{\Lambda}
\def\descsym{\desc_{\textsf{sym}}}
\def\gorder{\p}
\def\Gl{\G_1} %base group in the left 
\def\Gr{\G_2} %base group in the right
\def\Gt{\G_T} %target group
\def\GlGen{G} %default generator in \Gl
\def\GrGen{\hat{G}} %default generator in \Gr
\def\GtGen{G_T} %default generator in \Gr
\def\Gls{\Gl^*}
\def\Grs{\Gr^*}
\def\Gs{\G^*}


% operations
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\condProb}[2]{{\Pr}\left[\,#1\,|\,#2\,\right]}
\newcommand{\expect}[1]{{{\mathbf{E}}[{#1}]}}
\newcommand{\infi}[2]{\inf_{#1}\left\{#2\right\}}
\newcommand{\supr}[2]{\sup_{#1}\left\{#2\right\}}
\newcommand{\ceiling}[1]{\lceil #1\rceil}
\newcommand{\inner}[2]{\langle{#1,#2}\rangle}
\def\pprod{{\textstyle\prod}}
\def\ssum{{\textstyle\sum}}
\newcommand{\sfrac}[2]{{\textstyle\frac{#1}{#2}}}
\def\cross{\times}
\def\union{\cup}
\def\bigunion{\bigcup}
\def\intersection{\cap}
\def\bigintersection{\bigcap}
\newcommand{\concat}{{\,\|\,}}
\newcommand{\xor}{{\;\oplus\;}}
\newcommand{\OR}{{\textstyle\bigvee}}
\newcommand{\AND}{\;\wedge\;}
\newcommand{\eqdef}{\;\stackrel{\rm def}{=}\;}
\def\getsr{\stackrel{{\scriptscriptstyle\$}}{\leftarrow}}
\newcommand{\goesto}{{\rightarrow}}
\newcommand{\then}{{\;;\;\;}}  
\newcommand{\andthen}{{\;:\;\;}}
\def\suchthatt{\: :\:}
\newcommand{\suchthat}{{\mbox{s.t.\ }}}
\def\next{\,;\,}
\newcommand{\Colon}{{:\;\;}}


% games
\newcommand{\procfont}[1]{\mathsc{#1}}
\newcommand{\Initialize}{\procfont{Initialize}}
\newcommand{\Finalize}{\procfont{Finalize}}
\newcommand{\Onquery}[2]{\underline{\procfont{#1}(#2)}}
\newcommand{\InitializeCode}[1]{\Onquery{Initialize}{#1}}
\newcommand{\FinalizeCode}[1]{\Onquery{Finalize}{#1}}
\newcommand{\EncO}{\procfont{Enc}}
\newcommand{\DecO}{\procfont{Dec}}
\newcommand{\procLR}{\procfont{LR}}
\newcommand{\outputs}{\textrm{ outputs }}
\newcommand{\wins}{\textrm{ wins}}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\bad}{\mathsf{bad}}


% cryptosystems
\newcommand{\secpar}{\lambda}
\newcommand{\pk}{\mathsl{pk}}
\newcommand{\sk}{\mathsl{sk}}
\newcommand{\enc}{\mathcal{E}}
\newcommand{\keys}{\mathcal{K}}
\newcommand{\decc}{\mathcal{D}}
\newcommand{\advA}{A}
%\newcommand{\msg}{\mathsl{m}}
\newcommand{\ciph}{\mathsl{c}}
\newcommand{\coins}[1]{\mathsf{coins(#1)}}
\newcommand{\reject}{\bot}


% --- -----------------------------------------------------------------
% --- Specific Macros
% --- -----------------------------------------------------------------
\newcommand{\peq}{\ensuremath{\pi_{\mathsf{EQ}}}\xspace}
\newcommand{\pfe}{\ensuremath{\pi_{\mathsf{FE}}}\xspace}
\newcommand{\pab}{\ensuremath{\pi_{\mathsf{AB}}}\xspace}
\newcommand{\plr}{\ensuremath{\pi_{\mathsf{LR}}}\xspace}
\newcommand{\pconv}{\ensuremath{\pi_{\mathsf{2toQ}}}\xspace}
\newcommand{\pmul}{\ensuremath{\pi_{\mathsf{DM}}}\xspace}
\newcommand{\pmmul}{\ensuremath{\pi_{\mathsf{DMM}}}\xspace}
\newcommand{\pip}{\ensuremath{\pi_{\mathsf{IP}}}\xspace}
\newcommand{\pcomp}{\ensuremath{\pi_{\mathsf{DC}}}\xspace}
\newcommand{\pdecomp}{\ensuremath{\pi_{\mathsf{decomp}}}\xspace}
\newcommand{\ptclr}{\ensuremath{\pi_{\mathsf{TC-LR}}}\xspace}
\newcommand{\ptcab}{\ensuremath{\pi_{\mathsf{TC-AB}}}\xspace}

\newcommand{\feq}{\ensuremath{\mathcal{F}_{\mathsf{EQ}}}\xspace}
\newcommand{\ffe}{\ensuremath{\mathcal{F}_{\mathsf{FE}}}\xspace}
\newcommand{\fab}{\ensuremath{\mathcal{F}_{\mathsf{AB}}}\xspace}
\newcommand{\flr}{\ensuremath{\mathcal{F}_{\mathsf{LR}}}\xspace}
\newcommand{\fconv}{\ensuremath{\mathcal{F}_{\mathsf{2toQ}}}\xspace}
\newcommand{\fmul}{\ensuremath{\mathcal{F}_{\mathsf{DM}}}\xspace}
\newcommand{\fmmul}{\ensuremath{\mathcal{F}_{\mathsf{DMM}}}\xspace}
\newcommand{\fcomp}{\ensuremath{\mathcal{F}_{\mathsf{DC}}}\xspace}
\newcommand{\fdecomp}{\ensuremath{\mathcal{F}_{\mathsf{decomp}}}\xspace}
\newcommand{\fti}[1]{\ensuremath{\mathcal{F}^{\mathcal{D}_{#1}}_{\mathsf{TI}}}\xspace}
\newcommand{\ftclr}{\ensuremath{\mathcal{F}_{\mathsf{TC-LR}}}\xspace}
\newcommand{\ftcab}{\ensuremath{\mathcal{F}_{\mathsf{TC-AB}}}\xspace}



\newcommand{\s}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\env}{\ensuremath{\mathcal{Z}}\xspace}
\newcommand{\adv}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\F}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\alice}{\ensuremath{\mathsf{A}}\xspace}
\newcommand{\bob}{\ensuremath{\mathsf{B}}\xspace}
\newcommand{\shareq}[1]{\ensuremath{\llbracket{#1}\rrbracket_{_q}}\xspace}
\newcommand{\sharetwo}[1]{\ensuremath{\llbracket{#1}\rrbracket_{_2}}\xspace}

